SIEVE: Helping Developers Sift Wheat from Chaff via Cross-Platform Analysis

Software developers have benefited from various sources of knowledge such as forums, question-and-answer sites, and social media platforms to help them in various tasks. Extracting software-related knowledge from different platforms involves many challenges. In this paper, we propose an approach to improve the effectiveness of knowledge extraction tasks by performing cross-platform analysis. Our approach is based on transfer representation learning and word embeddings, leveraging information extracted from a source platform which contains rich domain-related content. The information extracted is then used to solve tasks in another platform (considered as target platform) with less domain-related contents. We first build a word embeddings model as a representation learned from the source platform, and use the model to improve the performance of knowledge extraction tasks in the target platform. We experiment with Software Engineering Stack Exchange and Stack Overflow as source platforms, and two different target platforms, i.e., Twitter and YouTube. Our experiments show that our approach improves performance of existing work for the tasks of identifying software-related tweets and helpful YouTube comments.

==> experiment.tex <==
\section{Experiments}
In this section, we describe the details of the setup of our empirical experiments. We first present the details of use cases. We then describe our experiment setting on the target domain/use cases.

\label{sec.experiment}
%\subsection{Dataset and Setting for Source Domain}

%For source domain, we use software engineering stack exchange data. Software Engineering Stack Exchange is a question and answer site for professionals, academics, and students working within the systems development life cycle. The dataset is publicly available on Stack Exchange data dump ~\footnote{http://archive.org/download/stackexchange}. We use the following two files: Posts.7z and Comments.7z. Posts.7z contains the title and body (i.e., question and answers) of posts that appear in StackExchange. Comments.7z contains comments that people give to the questions and answers in StackExchange. Our Stack Exchange dataset contains a total of 149,478 posts, 409,740 comments, and 46246 titles spanning from September 2010 to August 2017. We performed text pre-processing by removing HTML tags, replacing URL with \_URL\_, and removed all punctuation marks from the sentences in the titles, bodies, and comments. We also changed all words to their lower case.

%\subsection{Dataset and Setting for Target Domain}
%Our first use case attempt to improve a work by Sharma et al on finding software-relevant tweets. We use their dataset to make equal comparison. 
%The dataset consists of around 6,2 Million tweets downloaded through Twitter REST API. To collect tweets, they first obtained a set of microbloggers that are more likely to generate software related contents. They started with a collection of 100 seed microbloggers whoare well known-software developers. Next, they analyzed the follow links of these microbloggers to identify other microbloggers that follow or are followed by at least 5 seed microbloggers. After they had identified the target microbloggers, they downloaded tweets that are generated by these microbloggers. They conducted simple pre-processing on the collected tweets such as removing punctuation marks and URLs, and also changed all words into lowercase.
%\subsection{Evaluation Metrics}
%We manually inspect the top-K tweets that are returned by our model. We evaluate the effectiveness of our approach using accuracy@K. accuracy@K is defined as the proportion of tweets in the top-K positions that are software related. Accuracy@ K has also been used to evaluate other past studies [8] [8], [27], [29].
